Succinct Approximate Rank Queries

We consider the problem of summarizing a multi set of elements in $\{1, 2, \ldots , n\}$ under the constraint that no element appears more than $\ell$ times. The goal is then to answer \emph{rank} queries --- given $i\in\{1, 2, \ldots , n\}$, how many elements in the multi set are smaller than $i$? --- with an additive error of at most $\Delta$ and in constant time. For this problem, we prove a lower bound of $\mathcal B_{\ell,n,\Delta}\triangleq$ $\left\lfloor{\frac{n}{\left\lceil{\Delta / \ell}\right\rceil}}\right\rfloor $ $\log\big({\max\{\left\lfloor{\ell / \Delta}\right\rfloor,1\} + 1}\big)$ bits and provide a \emph{succinct} construction that uses $\mathcal B_{\ell,n,\Delta}(1+o(1))$ bits. Next, we generalize our data structure to support processing of a stream of integers in $\{0,1,\ldots,\ell\}$, where upon a query for some $i\le n$ we provide a $\Delta$-additive approximation for the sum of the \emph{last} $i$ elements. We show that this too can be done using $\mathcal B_{\ell,n,\Delta}(1+o(1))$ bits and in constant time. This yields the first sub linear space algorithm that computes approximate sliding window sums in $O(1)$ time, where the window size is given at the query time; additionally, it requires only $(1+o(1))$ more space than is needed for a fixed window size.

==> suffAlg.tex <==
\begin{algorithm}[]
	\caption{A \suff{} algorithm}\label{alg:suff}
	%\scriptsize
	%\begin{multicols}{2}
	\begin{algorithmic}[1]
		\State Initialization: $s \gets 0, o \gets 0, \ranker \gets \ssr.\text{init()}$
		\Function{\add[\text{element }\inputVariable]}{}
		\State $\blockOffset \gets (\blockOffset+1)\mod \blockSize$
		\State $s \gets s + Round_{\nBits}(x)$				\label{line:sum}
		%\Comment{Store $\bsFracInput$ using $\bsReminderFractionBits$ digits}
		\If {$\blockOffset = 0$}\label{line:end-of-block}
			\State $b \gets \floor{\frac{s}{\blockSize\cdot\bsrange}}$ \label{line:setBit}
			\State $s\gets s - \blockSize\cdot\bsrange\cdot b$ \label{line:reduceS}
			\State $\ranker.\mbox{\sc Add}(b)$
		\EndIf
		\EndFunction		
		\Function{Query}{$w$}
		\If{$w \le o$}
			\State \Return $s$
		\Else
			\State $\numBits \gets \ceil{\frac{w-o}{S}}$
			\State $\setBits \gets \ranker.\mbox{\sc Query}\parentheses{\numBits}$
			\State $\lastBit \gets \setBits - \ranker.\mbox{\sc Query}\parentheses{\numBits-1}$
			\State $\outBits \gets \outBitsVal$
			\State \Return {$\bsrange\cdotpa{S \cdot{\setBits}-\outBits\cdot \lastBit-S/2}+s + 1/2$}\label{line:est} \Comment{\footnotemark}
		\EndIf		
		\EndFunction
		
	\end{algorithmic}
	%\end{multicols}
\end{algorithm}
\footnotetext{While it may seem that the $1/2$ correction is unnecessary, this gives us an error that is \emph{strictly} lower than $\bserror$, which is required for the lower bound of~\cite{SWATPAPER}.}
